Finding the Right Place: Sensor Placement for UWB Time Difference of Arrival Localization in Cluttered Indoor Environments

Ultra-wideband (UWB) time difference of arrival (TDOA)-based localization has recently emerged as a promising indoor positioning solution. However, in cluttered environments, both the UWB radio positions and the obstacle-induced non-line-of-sight (NLOS) measurement biases significantly impact the quality of the position estimate. Consequently, the placement of the UWB radios must be carefully designed to provide satisfactory localization accuracy for a region of interest. In this work, we propose a novel algorithm that optimizes the UWB radio positions for a pre-defined region of interest in the presence of obstacles. The mean-squared error (MSE) metric is used to formulate an optimization problem that balances the influence of the geometry of the radio positions and the NLOS effects. We further apply the proposed algorithm to compute a minimal number of UWB radios required for a desired localization accuracy and their corresponding positions. In a real-world cluttered environment, we show that the designed UWB radio placements provide 47% and 76% localization root-mean-squared error (RMSE) reduction in 2D and 3D experiments, respectively, when compared against trivial placements.

==> sections/5-algorithm.tex <==
\begin{algorithm}[t]
% \small
\footnotesize
  \SetKwInput{KwData}{Input    ~}
  \SetKwInput{KwResult}{Output}
  \KwData{Number of anchor pairs $Q = m/2$, indoor space $\mathcal{P}$, possible anchor placement set $\mathcal{A}$, locations and materials of obstacles $\mathcal{O}$, pre-defined region of interest $\Phi \subset \left(\mathcal{P} \cap \mathcal{O}'\right)$, initial anchor positions $\Scale[1.0]{\bm{a}^{1}=\{\bm{a}^{1}_1,\cdots,\bm{a}^{1}_{m}\} \in \mathcal{A}}$, $k = 1$, and the maximum iteration max$_{\textrm{iter}}$.}
  \KwResult{Optimized placement $\Scale[1.0]{\bm{a}^{\star} \in \mathcal{A}}$.} 
  Select $N$ sample points $\mathbf{p}=\{\mathbf{p}_1,\cdots, \mathbf{p}_N\} \in \Phi$\; 
  \While{$k<\textrm{max}_{iter}$}{
    \For{$q\gets1$ \KwTo $Q$}{
        Select the $q$-th anchor pair $\{\bm{a}^{k}_i,\bm{a}^{k}_j\}_q$ \;
        Optimize $\{\bm{a}^{k\ast}_i,\bm{a}^{k\ast}_j\}_q$ to minimize the average RMSE over $\mathbf{p}\in \Phi$ in Equation \eqref{eq:mse_metric} \;
        Update the anchor pair $\{\bm{a}^{k}_i,\bm{a}^{k}_j\}_q \gets \{\bm{a}^{k\ast}_i,\bm{a}^{k\ast}_j\}_q$\;
    }
    $k \gets k+1$
  }
  \Return Optimized placement $\bm{a}^{\star}$ 
  \caption{\small BCM-based anchor placement algorithm}
\end{algorithm}
\section{Algorithm}
\label{sec:algorithm}
Given a general environment with known obstacles, applying the NLOS models constructed in Section~\ref{sec:tdoa_mm} to solve Equation~\eqref{eq:optimization_problem} is not trivial. %
In this work, we propose a block coordinate-wise minimization (BCM) algorithm~\cite{tseng2001convergence} to optimize Equation~\eqref{eq:optimization_problem}, which tends to be more efficient and scalable than solving the problem directly using nonlinear optimization solvers.
%
In the proposed BCM algorithm (see Algorithm~1), each anchor pair $\{\bm{a}_i, \bm{a}_j\}, (i,j)\in\Gamma,$ is treated as one coordinate block. At each iteration, we sequentially select one of the coordinate blocks and minimize the average RMSE $\mathcal{M}(\bm{a})$ w.r.t. the selected block while the other coordinate blocks are fixed. We use the \texttt{MultiStart}~\cite{matlab} solver provided by Matlab with $50$ random initial conditions for each optimization step (line~5 in Algorithm~1). 
%
In practice, operating the algorithm with a fixed number of iterations (max$_{\textrm{iter}}=5$), the algorithm typically converges to satisfactory placement solutions. 
%
Like for any general nonlinear optimization problem, we do not have guarantees for finding the global optimal solution, but our numerical solutions demonstrate significantly better performance in both simulation and experiments compared to trivial or intuitive anchor placements (shown in Section~\ref{sec:sim-exp}).

We further use the sensor placement optimization for localization system design. Given the obstacle positions, a pre-defined region of interest $\Phi$, and required localization accuracy $\mathcal{M}_r$, we propose an iterative algorithm based on Algorithm~1 to find a minimal number of anchors required to meet the accuracy $\mathcal{M}_r$ and their corresponding positions. Considering complicated indoor environments with solid walls and other obstacles, we constrain the anchor positions to the boundary of the indoor space. In each iteration, we optimize the anchor placement and add one extra pair of anchors if the desired localization accuracy is not satisfied. The positions of the extra anchor pair are initialised randomly on the boundary of the space. The algorithm terminates when the required accuracy is satisfied or no solution can be found with the maximum allowable number of anchors. The detailed localization system design algorithm is presented in the supplementary material\footref{fn:supplementary} (Algorithm~2).

==> sections/6-sim_exp_res.tex <==
\section{Simulation and Experimental Results}
\label{sec:sim-exp}
In this section, we present simulation and experimental results of the proposed sensor placement algorithm. The algorithm is implemented in Matlab and we use Bitcraze's Loco Positioning system (LPS) for experimental validation. We first demonstrate the performance of the proposed algorithm under different simulated conditions, which use the experimentally identified NLOS models. Then we apply the sensor placement algorithm to a real-world cluttered environment for both 2D and 3D settings. Optimized anchor configurations are obtained in simulation and we demonstrate the effectiveness of the designed placement through the improvement of real-world localization performance compared to trivial anchor placements. Finally, we discuss the difference between the theoretical analysis and the real-world localization performance. 

\subsection{Simulation Results}
We present the simulation results in 2D through heatmaps where lower RMSE is indicated with darker color. We first apply the BCM-based anchor placement algorithm (Algorithm~1) to a simple 2D setup, where the region of interest $\Phi$, represented by solid white dots, lies within common and metal obstacles. We allowed anchors to be placed anywhere in the non-obstacle area. 
%
Good localization performance can be achieved in this case and the optimized anchor configuration, shown in Figure~\ref{fig:sim_res}a, is not trivial. 
%
\begin{figure}[tb]
  \begin{center}
    \includegraphics[width=0.49\textwidth]{figures/figure3.pdf}
  \end{center}
  \caption{Simulation results for 2D scenarios. The anchors and sample points are indicated by colored and white dots, respectively, with anchor pairs indicated by the same color. Non-metal and metal obstacles are represented by light and dark gray boxes, respectively. The optimized anchor placements balance the effects of anchor geometry and NLOS measurement biases to improve localization performance. 
  }
  \label{fig:sim_res}
\end{figure}

We then demonstrate the performance of Algorithm~1 in more challenging conditions with sample points close to obstacles. As shown in the Figure~\ref{fig:sim_res}b, when the obstacle is non-metal, the algorithm balances the effects of NLOS errors and the anchor geometry. When the obstacle is metal (see Figure~\ref{fig:sim_res}c), considering the large NLOS errors induced by such obstacles, the algorithm avoids all NLOS conditions. In Figure~\ref{fig:sim_res}d, we add one extra sample point at $(2,2)$ behind the metal obstacle (highlighted with a red arrow). In this scenario, no anchor configuration can cover all the sample points while avoiding NLOS. The proposed algorithm sacrifices the localization accuracy at the sample points on the right so as to cover the extra sample point. 

\begin{figure}[!b]
  \begin{center}
    \includegraphics[width=0.4\textwidth]{figures/figure4.pdf}
  \end{center}
  \caption{UWB TDOA-based localization system design results. Solid walls are indicated as black boxes. Twelve anchors are required to meet an accuracy of $0.05$ meter average RMSE over the sample points (white dots).}
  \label{fig:system-design}
\end{figure}

Next, we demonstrate the performance of the proposed TDOA localization system design algorithm. We consider a robot navigation task in a complicated indoor environment with solid walls and various obstacles as shown in Figure~\ref{fig:system-design}. The goal is to design an UWB TDOA-based localization system to provide an accuracy of $0.05$ meter average RMSE over the pre-defined region (indicated by sample points), where the anchors are constrained to be placed on the boundary of the space and walls.
%
In this complex system design problem, an intuitive anchor placement is generally hard to come up with, especially for TDOA-based hyperbolic localization. Consequently, it is necessary to design the anchor placement through Algorithm~2.
%
As demonstrated in Figure~\ref{fig:system-design}, $12$ anchors are required to meet the accuracy requirement, leading to around $0.04$ meter average RMSE over the sample points.

Finally, we evaluate the optimization performance for different random initial anchor positions (20 initial conditions for each scenario in Figure~\ref{fig:sim_res}, 10 for the system design scenario in Figure~\ref{fig:system-design}). 
%
The simulation results show that the variation in the position accuracy due to the random initialization is a magnitude (millimeters) lower than the average position error (centimeter).  Additionally, the number of required anchor pairs computed by Algorithm~2 is the same among all the simulation runs. Detailed simulation results are provided in the supplementary material\footref{fn:supplementary}.

\begin{figure}[tb]
  \begin{center}
    \includegraphics[width=0.41\textwidth]{figures/figure5.pdf}
  \end{center}
  \caption{Optimized 3D anchor placement in a cluttered environment with one metal cabinet (black) and three non-metal obstacles. The tag and anchors are indicated by red and blue circles, respectively.}
  \label{fig:exp-photo}
\end{figure}

\subsection{Experimental Results}
To validate the sensor placement design in realistic settings, we conducted real-world experiments in both 2D and 3D. One metal cabinet and three non-metal obstacles were placed in a $6m\times7m\times2.65m$ indoor space as shown in Figure~\ref{fig:exp-photo}. We used DW1000 UWB modules from Bitcraze's LPS to set up the UWB TDOA-based localization systems. The UWB modules are configured in decentralized mode (TDOA3) and the ground truth positions are provided by a motion capture system comprising of ten Vicon cameras. Since the main focus of this work is the localization performance of a given sensor placement design, we use multilateration~\cite{fang1986trilater} as the position estimator in our experimental validation. In both 2D and 3D experiments, we placed an UWB tag at each sample point to collect UWB measurements. The low-cost DW1000 UWB radio is known to have LOS measurement biases related to the antenna radiation pattern~\cite{zhao2021learning}. Therefore, we first map the LOS biases at each sample point with no obstacles in the space. Then, for the UWB measurements collected in the presence of obstacles, we reject large multi-path outliers with measurement errors larger than one meter and compensate for the LOS biases. In practice, the LOS biases can be identified in a lab setting and are shown to be generalizable to other anchor settings~\cite{zhao2021learning}. 
Moreover, the effects of LOS biases for more advanced UWB systems are usually negligible. At each sample point, the tag position is computed through multilateration.


% Box plot
\begin{figure}[b]
  \begin{center}
   \begin{tikzpicture}
    \centering
    \node[inner sep=0pt, opacity=1] (anchor) at (0.0,0.0){\includegraphics[width=.48\textwidth]{figures/figure6.pdf}};
    \node[text width=2.5cm, black] at (-0.4, 1.2) {\small 2D Exp.};
    \node[text width=2.5cm, black] at (3.4, 1.2) {\small 3D Exp.};
    \end{tikzpicture}
  \end{center}
 \caption{Root-mean-square error (RMSE) of the multilateration results in both 2D and 3D experiments. The optimized anchor placements achieve around $46.77\%$ and $75.67\%$ RMSE reduction in 2D and 3D, respectively, compared to the trivial placements. }
  \label{fig:boxplot}
\end{figure}
In 2D experiments, we select a challenging region of interest between the obstacles (indicated by the red points in Figure~\ref{fig:experimental_results}a-c) for anchor placement design. Conventional anchor placement design either places anchors in the corner or uniformly distributes the anchors on the boundary of the space, which we refer to as trivial placement $\#1$ and $\#2$, respectively. We apply Algorithm~1 with trivial placement $\#1$ as the initial guess. The corresponding multilateration results for the trivial and optimized anchor configurations are shown in Figure~\ref{fig:experimental_results}a-c. It can be observed that the localization performance in the two trivial placements deteriorates greatly due to the presence of obstacles. With the optimized anchor configuration, we are able to achieve a localization accuracy of $0.058$ meters, which represents an average RMSE reduction of $51.01\%$ and $42.53\%$ compared to the trivial placements $\#1$ and $\#2$, respectively. 

For 3D experiments, we compare the localization performance of the anchor positions computed from Algorithm~1 and a trivial placement. We sample $32$ points at $1m$ and $0.7m$ height. The anchor placement is constrained to the boundary of the 3D space. The multilateration results of the trivial and optimized 3D anchor configurations are shown in Figure~\ref{fig:experimental_results}d-e, respectively. For the trivial 3D anchor placement, the multilateration results show large errors over the sample points. Using the trivial placement as initial guess for optimization, we achieved a $75.67\%$ improvement in the average RMSE (from $0.291m$ to $0.071m$) with the optimized anchor placement. The multilateration RMSE errors in both 2D and 3D experiments are summarized in Figure~\ref{fig:boxplot}. 
% bar plot
\begin{figure}[t]
  \begin{center}
    \begin{tikzpicture}
    \centering
    \node[inner sep=0pt, opacity=1] (anchor) at (0.0,0.0){\includegraphics[width=.48\textwidth]{figures/figure7.pdf}};
    \end{tikzpicture}
  \end{center}
  \caption{Simulation and experimental results in 2D (on the left) and 3D (on the right). The RMSE results in simulation and reality show similar trends.}
  \label{fig:barplot}
\end{figure}

% figure 8 with one figure
\begin{figure*}[t]
  \begin{center}
    \begin{tikzpicture}
    \centering
    \node[inner sep=0pt, opacity=1] (anchor) at (0.0,0.0){\includegraphics[width=.85\textwidth]{figures/figure8.pdf}};
    \end{tikzpicture}
  \end{center}
\caption{Multilateration results (light blue dots) in real-world experiments. The non-metal and metal obstacles are indicated as gray and teal boxes. The ground truth sample points are indicated as red points. The trivial anchor placements are selected in the corner (2D trivial placement $\#1$,~(a) and 3D trivial placement~(d)) and uniformly distributed on the boundary (2D trivial placement $\#2$,~(b)) of the space. The optimized anchor placements in 2D~(c) and 3D~(e) balance the effects of anchor geometry and NLOS measurement biases, leading to improved localization performance over selected sample points.}
\label{fig:experimental_results}
\end{figure*}

Finally, we compare the average RMSE values from simulation and real-world experiments for 2D and 3D anchor configurations in Figure~\ref{fig:barplot}. It can be observed that the simulation and experimental results show similar trends, verifying that our NLOS models capture the real-world effects reasonably well. In reality, there exist small multi-path measurements that cannot be easily distinguished and rejected, which degrade localization performance. Moreover, the imperfect models for the UWB NLOS measurements also cause gaps between simulation and reality. We observe that the optimized 3D anchor placement shows the smallest RMSE difference between simulation and experimental results. The reason is that the optimized 3D anchor placement nearly avoids all NLOS conditions and thus the model imperfection does not affect the simulation results.


